Latent Space Translation via Inverse Relative Projection

The emergence of similar representations between independently trained neural models has sparked significant interest in the representation learning community, leading to the development of various methods to obtain communication between latent spaces. "Latent space communication" can be achieved in two ways: i) by independently mapping the original spaces to a shared or relative one; ii) by directly estimating a transformation from a source latent space to a target one. In this work, we combine the two into a novel method to obtain latent space translation through the relative space. By formalizing the invertibility of angle-preserving relative representations and assuming the scale invariance of decoder modules in neural models, we can effectively use the relative space as an intermediary, independently projecting onto and from other semantically similar spaces. Extensive experiments over various architectures and datasets validate our scale invariance assumption and demonstrate the high accuracy of our method in latent space translation. We also apply our method to zero-shot stitching between arbitrary pre-trained text and image encoders and their classifiers, even across modalities. Our method has significant potential for facilitating the reuse of models in a practical manner via compositionality.

==> sections/0.draft.tex <==
% \section{Introduction}
% \section{Related works}
% \section{Method}
% \section{Experiments}
% \section{Conclusions}


Fixed Story: fare zero-shot stitching fra moduli pre-trained è possibile perché spesso scale does not matter in practice


Scale invariance:
  -  Distribuzione norme fra word2vec e fasttext. Generalizzabile: Mostriamo che diversi encoder hanno norme in uno specifico range, ma senza correlazione (al contrario degli angoli)
  - Train MLP su encoding al layer i su megamodello. Rescale a test-time su dati di test gli i-esimi encoding: funziona ancora.
  - Verifica se il layer i è invariante alle norme.
      - Train MLP su encoding finali di un megamodello.  Rescale a test-time su dati di test gli i-esimi encoding interni prima di farli proseguire: funziona ancora.
      - Verifica che il megamodello è robusto alle norme.
  - Figura1 con linea aggiuntiva: mostra che MLP allenati su embedding che contengono informazione solo nell'angolo sono robusti al cambio di scala ad ogni layer

  - Transformazione inversa relative2abs (pruning + augmentation + inversa):
      - Esperimenti sistentici su griglia 2D visualizzabili (e.g. quadrato che ruota ma non si piega)
      - Diffusione da matrice identita' a matrice ancore (subset of train data) random
      - Diffusione da matrice identita' a matrice random
      - Riusciamo a mappare da spazi i-dimensionali a j-dimensionali, con j >> i

Esperimenti di zero-shot stitching:
  - Settings:
     - Transformer {NLP} (dataset: TREC, N24NEWS, ...)
     - Transformer {vision} (dataset: cifar10, cifar100, cifar100 coarse, N24news, ...)
     - Resnet {vision} (dataset: cifar10, cifar100, cifar100 coarse, N24news, ...)
     - Multimodali Immagine-Testo (WIP)

  - Anchors improvement:
      - Anchors selection (random, ...): scegliere ancore migliori
      - Anchors pruning e augmentation (transfer identity, random (?), ...): stabilizzare inversa
      - Sottospazi!! (?)

% Problemi:
%   - Centrare a volte aiuta e a volte no. In base a cosa?
%   - Perche' abbiamo encoder/decoder scale-invariant?



% ------


% --- INTRO
% 1. Le NN (transformer or classficiatori allenati su transformer) tendono a essere scale-invariant (in practice?)
%   - Dimostrato da Figura 7 e 8 (e altre)
%   - (?) Possibile dimostrazione: allenare parametri con constraint che devono produrre solo features sferiche. SOno più veloci? (o applicazione)
%   - Critiche:
        % - Vale anche per MLP semplici su MNIST/CIFAR? 
        % - È la normalizzazione Layer norm nel transformer il solo motivo per cui sono invarianti alla norma
        % - Il Classificatore è allenato solo sul transformer, il quale non codifica info nelle norme e quindi il classificatore non le utilizza
        
% 2. Lo sono perchè la scale è difficile da sfruttare?
%   - Un encoding che si basa su angoli centrati in zero è lineramente separibile e quindi semplice, Fig.1.   
%   - Critiche:
        % - Forse anche lo scale encoding va fatto denso in fasce
        % - Dipende dalla soluzione delle critiche del punto 1. (è tutto dovuto alla normalizzaione oppure no?) 
        % - (!) Più hai semantica più sfrutti gli angoli?

% 2.5. Riassunto dei contributi

% --- Related
% - Nystrom?

% --- METHOD
% 3. L'essere invarianti alla norma E essere centrati, significa che importano solo gli angoli rispetto l'origine
%   - Banale.
%   - Bonus:
        % Siamo centrati secondo l'assunzione in \cite{relreps}

% 4. Le rapprsentazioni relative considerano solo l'angolo, visto che la norma non è importante possiamo anche rel2abs. Questo apre ad applicazioni fighe ed estremamente rilevanti.
%   - Dimostrato tramite formula o esperimento sintetico
%   - Critiche:
%       - Serve fare l'inversa è instabile.
%       - Considerazioni sulla struttura delle ancore e loro ortogonalità. 

% --- EXPERIMENTS
% 5. Zero-shot stitching without training on relreps 
%   - Possiamo fare zero-shot stitching fra encoder e decoder pre-allenati
%   - Con diversi tipi di anchors selection
%   - Critiche (limitations):
        % - Casi in cui non funziona possono essere giustificati in modo analitico su esempi giocattolo andando ad  analizzare la matrice delle ancore per cui l'esempio giocattolo non funziona. Possibilità:
            % - Matrice singolare
            % - Roba collineare
            % - ?

% 6. (?) training sferico, se è più efficiente a convergere
% oppure scomporre la matrice di pesi in rotation + scaling e si lascia solo rotation. Converge prima perche' e' meno noisy avendo tolto lo scaling che non serve?







% Old Story: Abbiamo osservato che nelle reti neurali in classificazione non conta la norma, quindi puoi fare stitching fra modelli preallenati







% Cosa sappiamo: :)
% - La norma non è una buona feature da usare
% - Sappiamo che i transfomer ignorano la norma e ficcano tutta l'informazione negli angoli
%
% - Sappiamo che gli MLP allenati su transformer ignorano la norma: 
%   - Esperimento con singolo decoder 
%   - (!) Sappiamo solo che MLP allenati su roba che codifica informormazioni negli angoli sanno ignorare la norma
%   - sappiamo che c'entra qualcosa il bias, ma non sappiamo cosa 
%
% - Sappiamo che è difficile sfruttare l'informazione codificata nella norma per un: MLP
% 
% - Sappiamo che alcuni spazi pre-allenati hanno tutti gli embedding in range di norma distinti ma ben separabili
%   - (!) non sappiamo su transformer diversi come si comportano
%
% - Sappiamo che è possibile ricostruire abs from rel in alcuni contesti
%   - Sappiamo che a meno di norma risulta essere banale
%   - Abbiamo esperimenti sintetici
%   - Abbiamo esperimenti reali su un singolo spazio
% 
% - È possibile fare stitching zero-shot senza allenare relativo:
%   - Abbiamo esperimenti su transfomer in diversi stili
%   - Abbiamo esperimenti su CV con rexnet e transformer
%   - (!) Baseline con allenamento relativo
%   - (!) Sottospazi!!
%










% NO: future work
% New Story: Osserviamo che in questi task e dataset il manifold dei dati rappresentato tramite angoli continene tutta l'informazione necessaria per risolvere il task




==> sections/7.supmat.tex <==
 
\begin{figure}[h]
    \centering
    \begin{overpic}[clip,width=1\linewidth]{figures/mockup/anchors-diffusion.png}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
        %
    \end{overpic}
  
    \caption{TBA  }
    \label{fig:anchors-diffusion}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{overpic}[clip,width=.5\linewidth]{example-image-a}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
        %
    \end{overpic}
  
    \caption{Something to show that we can reconstruct the absolute spaces starting from a relative one, using only the anchor set. Maybe a formula is better?}
    \label{?}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{overpic}[clip,width=1\linewidth]{figures/mockup/scale-invariance.png}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
        %
    \end{overpic}
  
    \caption{TBA {Luca: Aggiungere una riga con il rescaling per far vedere che uno si rompe l'altro no}}
    \label{fig:scale-invariance-synthetic}
\end{figure}


\paragraph{Word Embeddings scale}
The well-known word embeddings, FastText and Word2Vec, exhibit a scale-invariant behavior. As shown in \Cref{fig:norm-ranges}, there is a clear separation between the FastText and Word2Vec norms and no correlation between the norms of the same words represented in the two spaces. This observation suggests that in this case, there is no semantically relevant information encoded in the norms. These results indicate that the scale of the embedding does not play a significant role in the performance of these word embedding models.



\paragraph{Big models scale-invariance}
We observed that large pre-trained models, such as transformers and resnets, are robust to internal rescaling of the encodings. Although we do not have a clear explanation for this phenomenon, we hypothesize that normalization layers and the linear separability of the information encoded in the angles instead of the norms (as seen in \Cref{fig:norm-ranges}) may play a role.
In \Cref{fig:rescaled-layer-acc}, we demonstrate the invariance a large transformer exhibits when the rescaling injection is applied at different layers: surprisingly, when the rescaling surpasses a certain threshold, the performance difference becomes negligible.
These results further emphasize the robustness of these pre-trained models to the rescaling injection and suggest that the scale of the embedding is not a critical factor in their performance.

\begin{figure}[h]
    \centering
    \begin{overpic}[clip,width=0.48\linewidth]{figures/mockup/rescaled_layer_factor_name_rescaled_acc.png}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
        %
    \end{overpic}
    \hfill
    \begin{overpic}[clip,width=0.48\linewidth]{figures/mockup/rescaled_layer_factor_name_acc_diff.png}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
        %
    \end{overpic}
    \caption{TBA: \luca{ refactor the images to be horizontal that fit better the template}}
    \label{fig:rescaled-layer-acc}
\end{figure}
 

\paragraph{Decoder scale-invariance}
We surprisingly observed that even MLPs trained on top of big models learn to be invariant to the rescale injection, as shown in \Cref{fig:decoder-norm-invariance}. We have complete control over the MLPs and surely they should not be invariant to rescaling by construction. 

Overall, these observation provide the foundation that enable the zero-shot stitching between independently pre-trained neural components that we will explore in the next section.



 \begin{figure}[h]
    \centering
    \begin{overpic}[clip,width=1\linewidth]{figures/mockup/transformer-norm-invariance.png}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
        %
    \end{overpic}
  
    \caption{TBA transformer-norm-invariance}
    \label{fig:transformer-norm-invariance}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{overpic}[clip,width=1\linewidth]{figures/mockup/decoder-norm-invariance.png}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
        %
    \end{overpic}
  
    \caption{TBA decoder-norm-invariance}
    \label{fig:decoder-norm-invariance}
\end{figure}


\begin{table}
\centering
\caption{TBA}
\label{tab:cross-space-inversion}
\begin{tabular}{llrrr}
\toprule
   &    &  mono similarity &  multi similarity &  rec similarity \\
encoding lang & decoding lang &                  &                   &                 \\
\midrule
\multirow{4}{*}{en} & en &             1.00 &              1.00 &            0.97 \\
   & es &             0.00 &              0.99 &            0.93 \\
   & fr &            -0.02 &              0.99 &            0.70 \\
   & ja &             0.03 &              0.99 &            0.84 \\
\cline{1-5}
\multirow{4}{*}{es} & en &             0.00 &              0.99 &            0.97 \\
   & es &             1.00 &              1.00 &            0.94 \\
   & fr &             0.01 &              0.99 &            0.69 \\
   & ja &             0.00 &              0.99 &            0.84 \\
\cline{1-5}
\multirow{4}{*}{fr} & en &            -0.02 &              0.99 &            0.97 \\
   & es &             0.01 &              0.99 &            0.93 \\
   & fr &             1.00 &              1.00 &            0.70 \\
   & ja &            -0.02 &              0.99 &            0.84 \\
\cline{1-5}
\multirow{4}{*}{ja} & en &             0.03 &              0.99 &            0.97 \\
   & es &             0.00 &              0.99 &            0.93 \\
   & fr &            -0.02 &              0.99 &            0.69 \\
   & ja &             1.00 &              1.00 &            0.85 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{HuggingFace transformers used in \Cref{?} to for cross-lingual transfer.}
\label{tab:transformers-nlp}
\begin{tabular}{lll}
\toprule
Language & HuggingFace transformers name    & Encoding Dim \\
\midrule
English  & openai/clip-vit-base-patch32     & 768          \\
English  & bert-base-cased                  & 768          \\
English  & roberta-base                     & 768          \\
English  & xlm-roberta-base                 & 768          \\
English  & google/electra-base-discriminator                 & 768          \\
Spanish  & PlanTL-GOB-ES/roberta-base-bne   & 768          \\
French   & ClassCat/roberta-base-french     & 768          \\
Japanese & nlp-waseda/roberta-base-japanese & 768          \\
\bottomrule
\end{tabular}
\end{table}
